RoboExpand: A Real2Sim2Real Data Engine with Agentic Reconstruction and Multi-View Video Generation

Collecting real-robot demonstrations across varied layouts and visual conditions is costly. Simulation can broaden this coverage, but discrepancies in geometry, contact dynamics, and appearance often hinder sim-to-real policy transfer. We introduce RoboExpand, an agentic Real2Sim2Real data engine that expands a single real-robot demonstration into diverse action trajectories and visual observations for policy learning. A reconstruction agent first replays the recorded actions and uses discrepancies in contact and object motion to refine the scene's geometry and physics. A trajectory generalization agent then adapts the demonstrated motion to new object layouts by planning paths that account for the new object positions. For each successful trajectory, the engine's learned multi-view transfer model finally generates synchronized videos under different visual conditions, preserving alignment with the trajectory's actions and states. Across four tasks on three real robot platforms, with 80 demonstrations per task, policies trained on RoboExpand-generated data achieved an average success rate of 72.5%, up from 40.0% with raw simulator renderings and close to the 75.0% achieved with real demonstrations. In additional generalization experiments on two Astribot tasks, policies trained on synthetic data covering the five tested visual conditions achieved an average success rate of 68.0%, compared with 39.0% for policies trained on real demonstrations from the default scene.

==> resources/packages.tex <==
% For flexible citation formats (author-year, numeric)
\usepackage{natbib}

% For UTF-8 encoded CJK (Chinese, Japanese, Korean) characters
\usepackage{CJKutf8}

%\newcommandx
\usepackage{xargs}  

% todo notes
\usepackage{todonotes}  

% multirow
\usepackage{multirow}


% cref
\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}

% % using itemize
% \usepackage{enumerate}


\usepackage{subcaption}


\usepackage{svg}


==> tab/eva_500_summary.tex <==
% Main-paper summary; the full view-wise breakdown is in eva_500TestSet.tex.
% Values copied exactly from the supplied all-views rows.
\begin{table}[!htbp]
  \centering
  \caption{\textbf{Video generation quality on real-robot test episodes.} Generated videos are compared with real observations across 500 episodes and 1,424 matched views. Best results are in \textbf{bold}.}
  \label{tab:video_quantitative}
  \small
  \setlength{\tabcolsep}{2pt}
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
    \toprule
    Method & FID $\downarrow$ & FVD $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    Cosmos-Transfer2.5 & 65.616 & 906.624 & 10.818 & 0.4091 & 0.5770 \\
    Wan-Fun-Control & 17.815 & 333.984 & 15.764 & 0.6709 & 0.3136 \\
    RoboRender & 23.105 & 272.640 & 14.100 & 0.6068 & 0.4202 \\
    \textbf{Ours} & \textbf{6.415} & \textbf{65.961} & \textbf{21.340} & \textbf{0.7688} & \textbf{0.1862} \\
    \bottomrule
  \end{tabular*}
\end{table}

